The Limits of Pan Privacy and Shuffle Privacy for Learning and Estimation

There has been a recent wave of interest in intermediate trust models for differential privacy that eliminate the need for a fully trusted central data collector, but overcome the limitations of local differential privacy. This interest has led to the introduction of the shuffle model (Cheu et al., EUROCRYPT 2019; Erlingsson et al., SODA 2019) and revisiting the pan-private model (Dwork et al., ITCS 2010). The message of this line of work is that, for a variety of low-dimensional problems -- such as counts, means, and histograms -- these intermediate models offer nearly as much power as central differential privacy. However, there has been considerably less success using these models for high-dimensional learning and estimation problems. In this work, we show that, for a variety of high-dimensional learning and estimation problems, both the shuffle model and the pan-private model inherently incur an exponential price in sample complexity relative to the central model. For example, we show that, private agnostic learning of parity functions over $d$ bits requires $\Omega(2^{d/2})$ samples in these models, and privately selecting the most common attribute from a set of $d$ choices requires $\Omega(d^{1/2})$ samples, both of which are exponential separations from the central model. Our work gives the first non-trivial lower bounds for these problems for both the pan-private model and the general multi-message shuffle model.

==> main-family-old.tex <==
In order to apply Theorem~\ref{thm:main-lb} to a learning or optimization problem, we need a family of distributions $\{\bP_{v}\}$ such that $\| \{\bP_{v}\} \|_{\infty \to 2}$ is small and any accurate algorithm for the problem distinguishes $\bP_V^n$ from $\bU^n$. This subsection describes one such family we will use in most of our lower bound arguments.

Let $\cX = \pmo^d$ be the data domain.  Let $\bU_\cX$ denote the uniform distribution over $\cX$. For a parameter $\alpha \in (0,\nicehalf)$, a non-empty set $t \subseteq [d]$, and a bit $b \in \pmo^{d}$, we define the distribution $\bP_{d,t,b,\alpha}$ to be uniform on $\pmo^{d}$ except biased so that $\mathbb{E}_{x \sim \bP_{d,\alpha, t,b,\alpha}}(\prod_{i \in t} x_i) = 2\alpha b$. Its probability mass function is
\begin{equation} \label{eq:Ptb}
    \bP_{d,t,b,\alpha}(x) =
    \begin{cases}
        (1+2\alpha) 2^{-d} & \textrm{if $\prod_{i \in t} x_i = b$} \\
        (1-2\alpha) 2^{-d} & \textrm{if $\prod_{i \in t} x_i = -b$}
    \end{cases}
\end{equation}
Note that, by construction, for every non-empty $t' \neq t$, $\mathbb{E}_{x \sim \bP_{d,t,b,\alpha}}(\prod_{i \in t'} x_i) = 0$. In the case where $t=\emptyset$, we define $\bP_{d,t,+1,\alpha}$ and $\bP_{d,t,-1,\alpha}$ to be synonyms of $\bU_\cX$.

For dimension $d$, a parameter $k \leq d$, and $\alpha \in (0,\nicehalf)$, we define the family
\begin{equation} \label{eq:Pdk}
\cP_{d,k,\alpha} = \{ \bP_{d,t,b,\alpha} : t \subseteq [d], |t| \leq k, b \in \pmo \}
\end{equation}

\begin{rem}
$\cP_{d,k,\alpha}$ is a multiset that contains two copies of $\bU_\cX$ ($\bP_{d,\emptyset,+1,\alpha}$ and $\bP_{d,\emptyset,-1,\alpha}$).
\end{rem}

\begin{fact}
\label{fact:Pdk-size}
The size of the family $\cP_{d,k,\alpha}$ is $2\cdot \binom{d}{\leq k}$ where $\binom{d}{\leq k} = \sum_{j=0}^k \binom{d}{j}$.
\end{fact}

\begin{fact}
\label{fact:Pdk-mixture}
The uniform mixture over the family $\cP_{d,k,\alpha}$ is $\bU_\cX$
\end{fact}

The following lemma is implicit in many lower bounds for local differential privacy (e.g.~\cite{DuchiJW13,Ullman18,EdmondsNU20}), although we reprove it here for completeness.
\begin{lem} \label{lem:P-sample-bound}
    For every $d \in \N$, $k \leq d$, and $\alpha \in (0,\nicehalf)$,
    $$
        \| \cP_{d,k,\alpha} \|_{\infty \to 2}^{2} \leq \frac{4\alpha^2}{\binom{d}{\leq k}}
    $$
\end{lem}
\begin{proof}
Due to Fact \ref{fact:Pdk-mixture}, we can expand the definition of the $(\infty \to 2)$ norm as
\begin{align*}
\| \cP_{d,k,\alpha} \|_{\infty \to 2}^{2} &= \sup_{f \from \cX \to [\pm 1]} \sum_{\bP \in \cP_{d,k,\alpha}} \frac{1}{|\cP_{d,k,\alpha}|} \cdot \left( \ex{x \sim \bP}{f(x)} - \ex{x \sim \bU_\cX}{f(x)}  \right)^2 \\
    &= \sup_{f \from \cX \to [\pm 1]} \sum_{t\subseteq [d], |t|\leq k \atop b\in \{\pm 1\}} \frac{1}{|\cP_{d,k,\alpha}|} \cdot \left( \sum_{x \in \pmo^d } f(x)\cdot ( \bP_{d,t,b,\alpha}(x) - \bU_\cX(x)) \right)^2 \\
    &= \sup_{f \from \cX \to [\pm 1]} \frac{1}{2\binom{d}{\leq k}} \cdot \sum_{t\subseteq [d], |t|\leq k \atop b\in \{\pm 1\}} \left( \sum_{x \in \pmo^d } f(x)\cdot ( \bP_{d,t,b,\alpha}(x) - \bU_\cX(x)) \right)^2 \stepcounter{equation} \tag{\theequation} \label{eq:P-sample-bound-1}
\end{align*}
The final equality comes from Fact \ref{fact:Pdk-size}.
By definition, $\bU_\cX(x)=2^{-d}$ for any $x\in\pmo^d$. Also, note that \eqref{eq:Ptb} is equivalent to $\bP_{d,t,b,\alpha}(x) = (1 + 2\alpha b \cdot \prod_{i \in t} x_i)2^{-d}$. By substitution, we have
\begin{align*}
\eqref{eq:P-sample-bound-1} &= \sup_{f \from \cX \to [\pm 1]} \frac{1}{2\binom{d}{\leq k}} \cdot \left( \sum_{t\subseteq [d], 0<|t|\leq k \atop b\in \{\pm 1\}} \left( \sum_{x \in \{\pm 1\}^d } f(x)\cdot 2\alpha b \cdot \prod_{i \in t} x_i \cdot 2^{-d} \right)^2 + 2 \left( \sum_{x \in \pmo^d } f(x)\cdot ( 2^{-d} - 2^{-d} ) \right)^2 \right) \\
    &= \sup_{f \from \cX \to [\pm 1]} \frac{2\alpha^2}{\binom{d}{\leq k}} \cdot \sum_{t\subseteq [d], 0<|t|\leq k \atop b\in \{\pm 1\}} \left( \sum_{x \in \{\pm 1\}^d } f(x) \cdot \prod_{i \in t} x_i \cdot 2^{-d} \right)^2 \\
    &= \sup_{f \from \cX \to [\pm 1]} \frac{4\alpha^2}{\binom{d}{\leq k}} \cdot \sum_{t\subseteq [d], 0<|t|\leq k} \left( \sum_{x \in \{\pm 1\}^d } f(x) \cdot \prod_{i \in t} x_i \cdot 2^{-d} \right)^2 \\
    &\leq \sup_{f \from \cX \to [\pm 1]} \frac{4\alpha^2}{\binom{d}{\leq k}} \cdot \sum_{t\subseteq [d]} \left( \sum_{x \in \{\pm 1\}^d } f(x) \cdot \prod_{i \in t} x_i \cdot 2^{-d} \right)^2 \stepcounter{equation} \tag{\theequation} \label{eq:P-sample-bound-2}
\end{align*}
Define $\hat{f}(t) := \ex{X\sim \bU_\cX}{ f(X)\cdot \prod_{i\in t} X_i}$, the Fourier transform over the Boolean hypercube. This is precisely the term being squared above. So we have
\begin{align*}
\eqref{eq:P-sample-bound-2} &= \frac{4\alpha^2}{\binom{d}{\leq k}} \cdot \sup_{f \from \cX \to [\pm 1]} \sum_{t\subseteq [d]} \hat{f}(t)^2 \\
    &= \frac{4\alpha^2}{\binom{d}{\leq k}} \cdot \sup_{f \from \cX \to [\pm 1]} \ex{X\sim \bU_\cX}{f(X)^2} \tag{Parseval's identity} \\
    &\leq \frac{4\alpha^2}{\binom{d}{\leq k}}
\end{align*}
This concludes the proof.
\end{proof}

The following is an immediate corollary of Theorem \ref{thm:main-lb}, Lemma \ref{lem:P-sample-bound}, and Fact \ref{fact:Pdk-size}.

\begin{thm}
\label{thm:P-lb}
Let $\bP_{d,T,B,2\alpha}$ denote a distribution chosen uniformly at random from $\cP_{d,1,\alpha}$ (where $T$ is a uniformly random member of $\{\emptyset, \{1\},\dots,\{d\}\}$ and $B$ is a uniformly random member of $\pmo$). If $M$ is an $(\eps,\delta)$-pan private algorithm such that  $\delta \log\nicefrac {\binom{d}{\leq k}}{\delta} \ll \alpha^2 \eps^2  / \binom{d}{\leq k} $ and $\dtv(M(\bP_{d,T,B,\alpha}^n), M(\bU^n_\cX))$ is larger than a positive constant, %$M$ distinguishes $\bU^n$ from $\bP_V^n$ with constant probability,
	then
	$$
	n \geq \Omega\left(\frac{ \sqrt{\binom{d}{\leq k}} }{ \alpha \eps }\right)
	$$
\end{thm}

==> relationships.tex <==
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
\begin{center}
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da9980644252931874] 
\draw    (102,105) -- (496.5,105) ;
\draw [shift={(498.5,105)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-4.9) .. controls (6.95,-2.3) and (3.31,-0.67) .. (0,0) .. controls (3.31,0.67) and (6.95,2.3) .. (10.93,4.9)   ;
\draw [shift={(100,105)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-4.9) .. controls (6.95,-2.3) and (3.31,-0.67) .. (0,0) .. controls (3.31,0.67) and (6.95,2.3) .. (10.93,4.9)   ;

% Text Node
\draw (118,117) node [anchor=north west][inner sep=0.75pt]   [align=left] {local};
% Text Node
\draw (213,117) node [anchor=north west][inner sep=0.75pt]   [align=left] {shuffle};
% Text Node
\draw (313,117) node [anchor=north west][inner sep=0.75pt]   [align=left] {pan-private};
% Text Node
\draw (440,117) node [anchor=north west][inner sep=0.75pt]   [align=left] {central};
% Text Node
\draw (70,56) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{55.606892pt}\setlength\topsep{0pt}
\begin{center}
least power\\least trust
\end{center}

\end{minipage}};
% Text Node
\draw (457,56) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{55.459392pt}\setlength\topsep{0pt}
\begin{center}
most power\\most trust
\end{center}
\end{minipage}};
\end{tikzpicture}
\end{center}
